VideoCon: Robust Video-Language Alignment via Contrast Captions

Despite being (pre)trained on a massive amount of data, state-of-the-art video-language alignment models are not robust to semantically-plausible contrastive changes in the video captions. Our work addresses this by identifying a broad spectrum of contrast misalignments, such as replacing entities, actions, and flipping event order, which alignment models should be robust against. To this end, we introduce the VideoCon, a video-language alignment dataset constructed by a large language model that generates plausible contrast video captions and explanations for differences between original and contrast video captions. Then, a generative video-language model is finetuned with VideoCon to assess video-language entailment and generate explanations. Our VideoCon-based alignment model significantly outperforms current models. It exhibits a 12-point increase in AUC for the video-language alignment task on human-generated contrast captions. Finally, our model sets new state of the art zero-shot performance in temporally-extensive video-language tasks such as text-to-video retrieval (SSv2-Temporal) and video question answering (ATP-Hard). Moreover, our model shows superior performance on novel videos and human-crafted captions and explanations. Our code and data are available at https://github.com/Hritikbansal/videocon.

==> sec/old_intro.tex <==
\section{Introduction}
\label{sec:intro}

\textbf{Para 1}
\begin{enumerate}
    \item The long standing challenge for AI is robust semantic alignment of diverse data modalities. In this regard, we have 
    CLIP: Image-Text, VideoCLIP: Video-Text. ImageBind: Video-Image-Text. In addition, we have generative models such as mPLUG-Owl, LLaVA, PaLI-1/3, GPT4-V that can generate natural language outputs (e.g., Yes/No) to specify the alignment between data modalities. 
    \item Understanding the alignment between the data modalities fuels practical applications such as retrieval and question answering. 
    \item Specifically, alignment evaluation for video and text is quite challenging. video is complex: objects that perform actions in a temporal order, and much more. 
\end{enumerate}

\textbf{Para 2}
\begin{enumerate}
  \item Prior works \cite{gardner2020evaluating,ma2023crepe,yuksekgonul2022and,lu2023evaluation,yarom2023you} show that the image-text alignment models struggle with contrast captions either created by humans or machine-generated. \cite{park2022exposing} find that the video-text alignment models such as CLIP4CLIP are not robust to the perturbations in the entity and verb phrase in the original captions, and hence, suffer on the retrieval task.
  \item In this work, we propose \name, a holistic dataset for robust video-language alignment evaluation. Holistic: covers a wide range of plausible contrast sets spanning object, attribute, relations, count, action, hallucination, and event order. These misalignments are generated by LLMs cheaply in a scalable manner. \name (LLM) is constructed from the combination of \msr, \vatex, and \tempo dataset. \hb{will mention the dataset statistics} 
  \item Novel: (a) Comes with a train and test set. (b) Since humans often specify the misalignments between the data modalities through natural language explanations, we also equip our dataset with these to specify the difference between the original video and contrast caption (say ``the video shows two person playing football, not three"). Overall, each instance from \name consists: video, caption, contrast caption, and natural language explanation for the difference between video and contrast caption.
\end{enumerate}

\textbf{Para 3}
\begin{enumerate}
  \item Firstly, we identify temporally challenging instances in the \msr and \vatex datasets. Specifically, we utilize a SOTA image-text alignment evaluation model on SEETRUE benchmark,  \cite{yarom2023you}, to identify easy instances and temporally-challenging instances in \msr and \vatex datasets. Subsequently, we filter easy instances to retain challenging video-text instances before contrast caption generation. 
\item Then, we assign one of the seven possible contrasting misalignment to the captions. For instance, we ensure that the captions from the temporally-difficult instances that contain multiple events (e.g., a boy is \textit{throwing} a ball and the girl is \textit{catching} it) are assigned event flip misalignment. 
  \item Subsequently, we prompt PaLM-2 API (LLM) to create contrast captions and natural language explanations (e.g., a boy is \textit{catching} the ball while a girl is \textit{throwing} it). We perform further filtering to remove bad generations. We provide more details on the dataset filtering and contrast caption generation in \S \hb{add section number}.
\end{enumerate}

\textbf{Para 4}
\begin{enumerate}
\end{enumerate}

\textbf{Para 5}
\begin{enumerate}
    \item We further enrich the \name dataset with human-generated contrast captions for the videos in the ActivityNet dataset. Since \name (Human) is completely unseen for \model, we assess its ability to generalize out-of-distribution. 
    \item We find that \model outperforms the baseline model on \name (Human) by \hb{XYZ} AUC-ROC on entailment task. In addition, \model performs well on the natural language explanations too.
    \item Finally, we show that \model achieves SOTA results on the downstream tasks such as zero-shot text-to-video retrieval on temporally-challenging SSv2-Events and SSv2-Temporal and zero-shot video question answering on temporal-challenging ATP-Hard, by beating previous best numbers by \hb{A} mAP points and \hb{B}$\%$ accuracy, respectively. 
\end{enumerate}


